The iNaturalist Species Classification and Detection Dataset

Existing image classification datasets used in computer vision tend to have a uniform distribution of images across object categories. In contrast, the natural world is heavily imbalanced, as some species are more abundant and easier to photograph than others. To encourage further progress in challenging real world conditions we present the iNaturalist species classification and detection dataset, consisting of 859,000 images from over 5,000 different species of plants and animals. It features visually similar species, captured in a wide variety of situations, from all over the world. Images were collected with different camera types, have varying image quality, feature a large class imbalance, and have been verified by multiple citizen scientists. We discuss the collection of the dataset and present extensive baseline experiments using state-of-the-art computer vision classification and detection models. Results show that current non-ensemble based methods achieve only 67% top one classification accuracy, illustrating the difficulty of the dataset. Specifically, we observe poor results for classes with small numbers of training examples suggesting more attention is needed in low-shot learning.

==> iNat Dataset CVPR 2018/inat_figs/train_ims/train_ims.tex <==
\newcommand{\turnheightnew}{0.195\columnwidth}

\centering
\begin{tabular}{c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{\hskip 2pt}c@{}}
		{\rotatebox{90}{\hspace{8pt}Actino}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_174_3f431953f8ea4715962f256963d3df68.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_5058_7bece36c1cdfd0e8392a3607021a3c69.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_3288_38f5ed69f3d0d8bb4eb4058329768649.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_269_07e11f4f7832e3bbf47ec476df5d9988.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_5058_ebe4b1a8654ce0a2b1e2cf16dbbeeaf3.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_4430_94fe6b4028ee1d6cbf3411b20a8f07c5.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_539_9a3b25dbfe242c5214f83924e12d0c9b.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_4389_bab9c9ce30da4532901cfd3863dfd62c.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_3361_d2ae27187b7c7b3a928f89bdac6f42f6.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/0_2666_73aa31e65505a55e82175843adb60e6c.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Amphib}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_4152_a983790f31a087e7a371677dfec3484c.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_653_6490f390fee361c63f4e1e05b4d346e9.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_2391_93fa157f8dd7cce497958db17c941075.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_2877_e1397b1d0d8cbacc975176162fb2fefd.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_222_3974b49d51efc45de381cfe9ff722235.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_5055_e28e83f7e173d7fdc66ec8421622c187.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_1678_1b1cc98232b1b31d7d84241f8b12e1e7.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_4628_7e5e91c5c19a78b4d35f424b331dc6a3.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_4751_51a4aaf3276952348ab498d66a1c7c03.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/1_1972_88c483e80ed3f97b3344ac747cc77c3b.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Animal}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_2917_6546e43e5519a82e5bc293b1a42662ae.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_2719_43afa0fc9bbb487abff6709f1675ac9e.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_1688_0ff2145819a13220c2aba2e81c5e569e.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_2883_46fc91cb0ddb71332f2a512261d92b4b.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_1688_759d1968217afdceeca25d1f9ca7767f.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_1847_37c4561e32fdfdca561e425955df7d30.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_3028_4731c509408c1b6b9e716d7e17faca55.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_4263_b758533bec4a1f8b4a7a9111409e6880.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_4083_95c831861db7ad5fd7d9f6de4d4df67d.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/2_1688_a902bf73a76596993819772e48349ed8.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Arachn}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_506_b00f1e9b52781ce2cdd6c72c69120096.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_4879_61a8a6205ee9708f4fb8671c73345851.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_3798_637ee4568157d4da7a7d3812f1389755.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_4519_4cfc5f9649656e037b964a2aa53bfdcf.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_3951_7a3d1a0a03969ce2d5de49d00ef3b3c5.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_3414_f9543a985454559a33ac42a91a1f2257.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_4519_fdb11233f8cfcb882e4c52b0250adcdf.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_4180_f180de881fb6defbfed5911cdf1dcf6c.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_4519_4167cc0ffd3e8a99ad896736fa1b3b68.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/3_605_98d4cf5c0f83f2cee7854348bb5600c4.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Aves}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_166_fe495b825297116ec227624c509ad435.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_4812_8d6faef03b9bcc883de0ef1ddf978c18.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_4311_a360aa674279dba5cf5efb4f0671dde9.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_4688_0731621c24b2239c1aa51b7e5b229f3e.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_2879_78c1617eb104f60ed988ec670e189681.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_2906_7510a9e2e8e06da7972f94f2723fea5a.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_2837_c5d86177dc490f9c85efa49a8783b952.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_963_c5b22f4093fd25e84217c003bb350b65.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_4281_b49e6af1a2307a3fc8aeb2cf14bbd668.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/4_1096_b9140eb270c17cd43187909cb36b8c74.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Chromi}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_4089_12ca2bbb885d7d8a72d490e310334cde.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_1559_7ac72251354494409d783faddda0c94b.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_3575_ce4e2fc6ee43dee131c37d072d7a13db.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_1559_6452662c973a523067d668de3d58074e.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_3575_2b4f54036f362dc51ced4ea3783d59ca.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_1113_d57d5a0841d7808d29fbfb5391ccfc8f.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_2628_ba83ca4aae7eb36a27207f47af4a1b5a.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_4089_33e5f7097e063c84aea6d22180112af2.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_1214_501072c2a5418b7e06367285b57b50dd.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/5_1327_7bbcdb1e94b81ea40afdf49f107342a4.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Fungi}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_4175_b05902e9a0c52897b9624fca420d16fd.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_3155_17c7577334f43bc7829fa5b46bd3d8c2.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_411_af034267323e0f0d53e606477a54061f.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_4409_bd56204cf282f50d33dac2bcf18c807e.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_3080_61682d288ab1b206445c87c2747d9428.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_1193_e51209c2be751d6eab0ddc26a1d2eb05.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_1211_5a4dff7a87015957131e9f450bb07160.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_4073_ee8f705ea6e4bc9cae1ecbe2c2679a58.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_412_33d1faf634705bffa25a8510ba2658d2.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/6_3044_1280278ef9e0a7268831f85e5244d555.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Insect}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_4785_03dfc85ca6c50c0196789100fa8ddc72.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_2993_d1f483d458a94abae3aba25479b48ec3.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_2901_93d820b06c079e46813b1ee52f3b1365.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_4200_5a7f1fb285ebfe768ab95eb459e3b275.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_1375_03bf7f624f82597502d7f674c2822c7d.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_1777_eccf2da2d708a24db1ca63b205029b16.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_4054_25b1ff00864e52a050b10070f191444a.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_4828_aeea7ab8b057ee24da493176b96c7d50.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_1730_6b9dc195207b894e4636a8efe8c604df.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/7_4199_09bc5c0aea4a73a581dc082cd0449a5b.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Mammal}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_1505_af1986bec985b45f0f35aac9f80fb863}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_642_de47c99860ec1c538eae3fa74950ee89.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_4492_e1dd0051c6d5b84f965f68ced5db18d2.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_3406_32af7139fd56b1d1eabd8ccf5e490c9f.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_1505_5dee4bb0e6b02a8bf296c31fe9a417e4.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_2566_3cac73b138de561c82c368cce23913ea}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_4614_ab4d2c555d73cacce00ace5d692c833a.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_4492_37cadb8c6077714c115654be9c1ab853.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_99_ebb6720ce755222f371450f1b4f17654.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/8_4410_fc6ffadd437da3841ad1bf3a46aba822.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Mollus}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_5080_cba6dbd12def7b86a2f522c436344ca6.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_2135_3ed3fbb1bc54f8940c493df71dd76536.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_4033_dc2a62c722ddc703cf10a85428672d71.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_2665_db046946d63dc22c407df911a2f7c170.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_4612_a72fa3442f99555aa13ddf786309ba56.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_1446_f744587452389a974205c18228354c01.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_1003_8d8a5109c111d963d501cd59ef89c92e.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_4356_1be1bce38645e18db4e3722b9e7d5ca9.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_4594_eed25f51fa16174ad8fd0f9163406f8c.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/9_284_53207bbde342d943f30daf2a6526a8c4.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Planta}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_4661_95d2073c0b84fc8e08ab1a800d6165df.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_248_59db085475bc0573bf409116b50ab909.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_2283_65885ce9a8edea86571b565af8f9c95d.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_1504_13e28289ef249e0e968f98524c4102a9.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_3637_01b9931ea78a5a303c622e8da3f601eb.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_4101_22ee10666968746c5b52df54ff46ac76.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_4437_377fc363e540108fe24495b73685b45f.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_1397_630cf59b925da644b319d1c3e4ecfe07.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_892_10b5bf5097fb29bc2bea8c6f5eb46141.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/10_651_ba39719f0646ba4395b29319b2ab36d5.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Protoz}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4145_ad37acea3843defee4dc399b7b1a191d.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4921_a48cca79e7c6d19d4c56121a9caafa27.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_1785_65d04bb6ed23ac6c99316fa3f628b0f9.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4145_11636e99e041c314fa48a1247acf48d4.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4921_ecd5c4f5d76381dcea013e0e4ffd94ff.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4921_e9870df8e103700239788c4adccde8e6.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4145_848a228b19004feb294fb6e60c4c8e8b.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4921_d1683e1cfc511b6dcb051c25c0493352.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_3861_249a1de093e5331edd5f2c4619786c5d.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/11_4145_e99d09bd67a508903248f6a3cb8cecd6.jpg}\\
		{\rotatebox{90}{\hspace{8pt}Reptil}} 
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_4231_76da04ffcc02313fff802ef53412e851.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_4864_1cdbd5731d8ea909dbc5ed689f2f5b1c.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_2023_e68a28c7a685b9df048cdd422fe472de.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_2392_75971f8f5750341daa808acaacd9d129.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_488_ff3d9bda1b04b0f2857ff1999c2ee159.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_1161_096b3a75b12f36bbd04a7527e45774e5.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_2562_d011ae5f557f66bd097e5494dfd1c831.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_4314_cc71859f39191e880f9cbdc6ec824a11.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_3108_7892360d012980d4152ccaddb87f401b.jpg}
		 & \includegraphics[height=\turnheightnew]{inat_figs/train_ims/train_ims/12_4558_61293f916013b6fa4df0f1990cd265cc.jpg}\\
\end{tabular}


